SLaDe: A Portable Small Language Model Decompiler for Optimized Assembly

Decompilation is a well-studied area with numerous high-quality tools available. These are frequently used for security tasks and to port legacy code. However, they regularly generate difficult-to-read programs and require a large amount of engineering effort to support new programming languages and ISAs. Recent interest in neural approaches has produced portable tools that generate readable code. However, to-date such techniques are usually restricted to synthetic programs without optimization, and no models have evaluated their portability. Furthermore, while the code generated may be more readable, it is usually incorrect. This paper presents SLaDe, a Small Language model Decompiler based on a sequence-to-sequence transformer trained over real-world code. We develop a novel tokenizer and exploit no-dropout training to produce high-quality code. We utilize type-inference to generate programs that are more readable and accurate than standard analytic and recent neural approaches. Unlike standard approaches, SLaDe can infer out-of-context types and unlike neural approaches, it generates correct code. We evaluate SLaDe on over 4,000 functions from ExeBench on two ISAs and at two optimizations levels. SLaDe is up to 6 times more accurate than Ghidra, a state-of-the-art, industrial-strength decompiler and up to 4 times more accurate than the large language model ChatGPT and generates significantly more readable code than both.

==> discussion.tex <==
\section{Discussion}
\label{sec:dis}

\paragraph{Code readability of decompiled functions} As shown in the example diagram and in the edit distance results, our model obtains decompilations that are lexically closer to the original function than ghidra. While a great this of this difference comes from the fact that our decompiler can predict meaningful variable names as opposed to placeholder names, the expressions, structure and statements are also more readable. For instance, ghidra introduces many casts that make functions practically impossible to follow, and pointer variables are treated as long integers, without being obvious the underlying type of the pointed object.

\paragraph{Decompilation errors due to missing dependencies} A great deal of decompilation errors of our models in Anghabench seems to come from an inherent difficulty of the way it is evaluated: in inference time, the model can correctly predict a decompilation using a given auxiliary type. However, this was not the type used in the original compilation, the type definition is not available in inference time, and thus the resulting C can't be executed or even compiled. We believe this kind of errors should be fixable without fundamentally changing the model itself, but coupling it with some additional mechanism.

\paragraph{On the readability-accuracy trade-off of decompilation} There seems to be a trade-off between readability and accuracy of decompilers. Neural methods typically produce more readable code than rule-based systems, at the expense of not being so reliable in obtaining actually executable C code. However, we have shown that it is possible to make neural systems way more accurate without sacrificing readability, situating the approach in the sweeter spot of the trade-off.

\paragraph{Towards practical neural decompilation} We the obtained results, our model sets the grounds towards practical neural decompilation that can actually be used out of the box.

\paragraph{Bidirectional model} We have shown that it is possible to build a bidirectional model without sacrificing performance. Our model is able to accurately compile quite sophisticated C functions.

\begin{comment}
\section{Related Work}

\subsection{Neural approaches}

%Synthetic setuo

Existing approaches frequently suffer from non-availability of models/data and synthetic
data.
In \cite{cao2022boosting}, binary is lifted to an intermediate representation and shown to perfrom well compared to the open-source decompiler RetDec.  However the evaluation was confined to  synthetic C programs containing only integer variables, no control-flow and simple arithmetic. Accuracy was 
defined as the number of  manually inspected correct basic blocks correct as opposed to IO equivalent programs. Furthermore, the RetDec evaluation is at odds with the large scale evaluation of \cite{liu2020far} (which shows much higher RetDec accuracy) due to  inaccuratley formatted inputs
In contrast in evaluating Ghidra, we ensure code entry points are clearly marked and provide
additional context to provide a fair comparison.

An alternative evolutionary approach based on genetic algorithms is explored in
\cite{schulte2018evolving} where IO accyracy is evaluated q. Here, snippets of exisiting code are combined and compiled and compared to the source binary. Unfortunately, this was evaluated on a small 19 
benchmark suite where  tens of thousands of evalutions are necessary to achieve approximately 50\/% accuracy 

While neural approaches have been poor at generating correct code, they have been more successful at generating accurate identifiers relative to anaytic approaches. In \cite{lacomis2019dire}
an encoder decoder LSTM model is used to determine variable names once an abnaltuc pass is used to 
decompile.


\subsection{LLMs as a programming tool}

Large language models have a  remarkable performance across a wide range of tasks.
In \cite{kashefi2023chatgpt},  chatGPT  can generate numerical method code in a number of programming languages.
In a more extensive evaluation \cite{austin2021program}, LLMs are shown to provide high accuracy
for a wide range of text to  program language tasks.
In \cite{sobania2023analysis}, chatGPT is shown, in a small scale experiment to ouperfrom existing program repair approaches. It, however, requires carful hints to ouperform existing deep learingning techniques \cite{prenner2022can,lutellier2020coconut}. Our evaluation goes against this finding and shows that decompilation is a more complex task for whuich small specialised models outperfrom massive general LLMs.. 


\subsection{Analytic decompilation}
% Hard to read
% Cannot infer out of context types and functions

Analytic approaches while highly accurate are often developed in the context of reverse engineering
understanding rather than as producng high level programs that are themselves
compilable objects. In  \cite{liu2020far}, an extensive evaluation  of decompilation correctness is presented focussing on 2 state of the art commercial and open-source compilers
where Ghidra is considered one of the best open-source decompilers. Ghidra is reported to have 
less than 10\% decpmpilation errors, smaller than our evaluation. However, the programs contain just one function, similar therefroe in complexity to our synthetic benchmark suite and no compiler optimizations. They not the difficulty of all tools in  infering out of context types.  

The poularity of LLVM withn the compiler community has seen research into lifting binaries to LLVM IR to enable retargetting to new ISA and hnce bonary translation \cite{yadavalli2019raising}. However as shown in \cite{liu2020far}, such approaches are insuffieceint for decompilation as they are unable to recover loval variabel names and high-level  control-flow structure. 

\subsection{Decompilation Correctness}
In this paper we use equivalence modulo inputs (EMI) testing \cite{} to test correctness.
In \cite {dasgupta2020scalable} a more rigorous approach is developed where translations are validated based on isomprphic graph matching, avoiding the need for theorem provers. 
EMI can be used as a cost-effective pre-processor for suach an approach. 
Binary decompilers such as Ghidra  use an external disassembler as a starting point.
Recent work \cite{verbeek2022formally} is able to verify the correctness of this fundamental 
starting point.

\end{comment}


==> extra_train.tex <==



We pose neural decompilation as a sequence-to-sequence task. Given a dataset $\mathcal{D}$ with $n$ pairs $\{(\mathbf{c_i}, \mathbf{s_i}) | i \in \{0..n-1\}\}$, where $\mathbf{s_i}$ is a function assembly code and $\mathbf{s_i}$ is the corresponding C code that produced it, we want to train a model T parameterized by $\bm{\theta}$ with maximum likelihood estimation:

\begin{align*}
\bm{\theta}^{*} = \arg\max_{\bm{\theta}} \prod_{i=0}^{n-1} P(\mathbf{c_i} | \mathbf{s_i}; \bm{\theta})
\end{align*}

In practice, we minimize the negative log-likelihood, which is equivalent to (multiclass) cross-entropy. For each minibatch (i.e., group of $K$ examples in the dataset), we use stochastic gradient descent to update the parameters of the model given the gradient of the cross-entropy loss function:

$\begin{aligned} \\ & \boldsymbol{P}(\boldsymbol{\theta}) = \operatorname{T}\left(\boldsymbol{z}_n, \boldsymbol{x}_n \mid \boldsymbol{\theta}\right) \\ & \operatorname{loss}(\boldsymbol{\theta})=-\sum_{t=1}^{\ell-1} \log P(\boldsymbol{\theta})\left[x_n[t+1], t\right] \\ & \boldsymbol{\theta} \leftarrow \boldsymbol{\theta}-\eta \cdot \nabla \operatorname{loss}(\boldsymbol{\theta})\end{aligned}$

%\begin{align*}
%\bm{\theta}^{*} = \arg\max_{\bm{\theta}} \sum_{i=0}^{n-1} \log P(\mathbf{c_i} | %\mathbf{s_i}; \bm{\theta})
%\end{align*}
%we are aiming to produce, 

%\begin{align*}
%\ell(\bm{\theta},\mathbf{D}) = -\sum_{(\mathbf{s_i},\mathbf{c_i}\in \mathbf{D})} \ln  %p(\mathbf{c_i}|\mathbf{s_i},\bm{\theta})
%\end{align*}




%\begin{align*}
% CE = -\sum_{t=1}^{\ell-1} \log P(\vth)[x_n[t\!+\!1],t]\
%\end{align*}


%\begin{align*}

%P = \vth - \eta \cdot \nabla \t{loss}(\vth) 
%C = -\frac{1}{N} \sum_{i=1}^{N} \sum_{j=1}^{C} y_{ij} \log(\hat{y}_{ij})
%\vth = \vth - \eta \cdot \nabla \t{loss}(\vth) 
%\end{align*}

\begin{comment}

Where:

LL is the cross entropy loss.
NN is the number of data points in the batch.
CC is the number of classes.
y_{ij}y 
ij
  is the true label (0 or 1) for class jj of data point ii.
\hat{y}_{ij} 
y
^
  
ij
  is the predicted probability for class jj of data point ii.
\end{comment}

%We take a training dataset $\mathcal{D}$
%which has $n$ pairs $\{(c_i, s_i) | i \in \{0..n-1\}\}$ with C (the $c_i$) and
%corresponding assembler
%(the $s_i$).  We train using
%the max-likelihood estimation:

%\begin{align*}
%\ell (\theta,\mathcal{T}) = \sum_{(c_i,s_i\in \mathcal{T})} \ln %P(c_i|s_i,\theta)
%\end{align*}

The transformer is parameterized by $\bm{\theta}$. We initialize the parameters from $\mathcal{N}(0, 0.02)$. Then, we optimize for $E$ epochs, for each batch 



%To train using this loss function
%we tokenize the data for use
%in a sequence-to-sequence transformer and

%{\em MOB how does cross-entropy fit here? This is a guess -please check!}
%We use cross-entropy as a measure of accuracy
%when adjusting. Simply put this is the normalized sum  of how many predicted C tokens at a position $i$ are equal to the ground-truth at position $i$ and is between 0.0 and 1.0.

 %{\em MOB again a guess!}
%A better measure is how IO accurate the predicted  sequence relative to ground truth, but
%compile and execute within a training loop would be excessively expensive. Edit-similarity, would be cheaper, but like IO accuracy is a non-differentiable metric and cannot be used in
% gradient-descent based training. Non-differentiable metrics require reinforcement based learning which while potential more accurate are expensive.
 
 
\begin{algorithm}[h] 
    \caption{$\hat{\vth}\gets$~\texttt{EDTraining}($\v{z}_{1:N_\t{data}}, \v{x}_{1:N_\t{data}},\vth$)}
    \label{algo:EDTraining_}
    \DontPrintSemicolon
    \tcc{Training a seq2seq model}
    \KwIn{$\{ (\v{z}_n, \v{x}_n) \}_{n=1}^{N_\t{data}}$, a dataset of sequence pairs.}
    \KwIn{$\vth$, initial transformer parameters.}
    \KwOut{$\hat{\vth}$, the trained parameters.}
    %\KwHyper{$N_\t{epochs} \in ℕ,\ η \in (0,∞)$}
    \KwHyper{$N_\t{epochs} \in \mathbb{N}, \eta \in (0,\infty)$}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \For{$i = 1, 2, \dots, N_\t{epochs}$}{
        \For{$n = 1, 2, \dots N_\t{data}$}{
            $\ell \gets \t{length}(\v{x}_n)$ \;
            $ \m{P}(\vth) \gets \texttt{EDTransformer}(\v{z}_n, \v{x}_n | \vth)\!\!$ \;
            $\t{loss}(\vth) = -\sum_{t=1}^{\ell-1} \log P(\vth)[x_n[t\!+\!1],t]\!\!$ \;
            %$\vth \gets \vth - η \cdot \nabla \t{loss}(\vth) $ \;
            $\vth \gets \vth - \eta \cdot \nabla \t{loss}(\vth) $ \;
        }
    }
    \Return $\hat{\vth} = \vth$

\end{algorithm}


==> final_plots/correlations_Synth.tex <==
\begin{table}
\caption{Synth feature correlations}
\thnormal
\begin{tabular}{lrrrrrrrrrrrr}
 & \multicolumn{3}{r}{ARM_O0} & \multicolumn{3}{r}{ARM_O3} & \multicolumn{3}{r}{x86_O0} & \multicolumn{3}{r}{x86_O3} \\
 & ChatGPT  & GHidra  & Slade  & ChatGPT  & GHidra  & Slade  & ChatGPT  & GHidra  & Slade  & ChatGPT  & GHidra  & Slade​ \\
compiles & \background-color#f59f80 \color#000000 \text-aligncenter 0.48 & \background-color#d65244 \color#f1f1f1 \text-aligncenter 0.80 & \background-color#d0473d \color#f1f1f1 \text-aligncenter 0.84 & \background-color#f7af91 \color#000000 \text-aligncenter 0.39 & \background-color#c12b30 \color#f1f1f1 \text-aligncenter 0.93 & \background-color#e97a5f \color#f1f1f1 \text-aligncenter 0.65 & \background-color#f7aa8c \color#000000 \text-aligncenter 0.41 & \background-color#d44e41 \color#f1f1f1 \text-aligncenter 0.82 & \background-color#d75445 \color#f1f1f1 \text-aligncenter 0.79 & \background-color#f39475 \color#000000 \text-aligncenter 0.53 & \background-color#c12b30 \color#f1f1f1 \text-aligncenter 0.93 & \background-color#e57058 \color#f1f1f1 \text-aligncenter 0.68 \\
edit_sim & \background-color#edd2c3 \color#000000 \text-aligncenter 0.13 & \background-color#efcfbf \color#000000 \text-aligncenter 0.16 & \background-color#f2cab5 \color#000000 \text-aligncenter 0.21 & \background-color#f1ccb8 \color#000000 \text-aligncenter 0.19 & \background-color#f4987a \color#000000 \text-aligncenter 0.50 & \background-color#eed0c0 \color#000000 \text-aligncenter 0.16 & \background-color#efcfbf \color#000000 \text-aligncenter 0.16 & \background-color#e3d9d3 \color#000000 \text-aligncenter 0.05 & \background-color#f4c6af \color#000000 \text-aligncenter 0.24 & \background-color#f1ccb8 \color#000000 \text-aligncenter 0.19 & \background-color#f5c2aa \color#000000 \text-aligncenter 0.26 & \background-color#f7b396 \color#000000 \text-aligncenter 0.36 \\
asm_length & \background-color#d5dbe5 \color#000000 \text-aligncenter -0.06 & \background-color#cfdaea \color#000000 \text-aligncenter -0.09 & \background-color#b6cefa \color#000000 \text-aligncenter -0.27 & \background-color#cfdaea \color#000000 \text-aligncenter -0.10 & \background-color#abc8fd \color#000000 \text-aligncenter -0.32 & \background-color#cedaeb \color#000000 \text-aligncenter -0.11 & \background-color#bcd2f7 \color#000000 \text-aligncenter -0.23 & \background-color#d9dce1 \color#000000 \text-aligncenter -0.02 & \background-color#c6d6f1 \color#000000 \text-aligncenter -0.16 & \background-color#cedaeb \color#000000 \text-aligncenter -0.10 & \background-color#b7cff9 \color#000000 \text-aligncenter -0.25 & \background-color#b5cdfa \color#000000 \text-aligncenter -0.27 \\
c_length & \background-color#cdd9ec \color#000000 \text-aligncenter -0.11 & \background-color#d4dbe6 \color#000000 \text-aligncenter -0.06 & \background-color#b6cefa \color#000000 \text-aligncenter -0.26 & \background-color#e0dbd8 \color#000000 \text-aligncenter 0.03 & \background-color#cbd8ee \color#000000 \text-aligncenter -0.13 & \background-color#cad8ef \color#000000 \text-aligncenter -0.14 & \background-color#c4d5f3 \color#000000 \text-aligncenter -0.17 & \background-color#dcdddd \color#000000 \text-aligncenter -0.00 & \background-color#c1d4f4 \color#000000 \text-aligncenter -0.19 & \background-color#d4dbe6 \color#000000 \text-aligncenter -0.07 & \background-color#c6d6f1 \color#000000 \text-aligncenter -0.16 & \background-color#b5cdfa \color#000000 \text-aligncenter -0.27 \\
n_fun_args & \background-color#c0d4f5 \color#000000 \text-aligncenter -0.20 & \background-color#c1d4f4 \color#000000 \text-aligncenter -0.19 & \background-color#bed2f6 \color#000000 \text-aligncenter -0.22 & \background-color#dadce0 \color#000000 \text-aligncenter -0.02 & \background-color#b6cefa \color#000000 \text-aligncenter -0.27 & \background-color#c4d5f3 \color#000000 \text-aligncenter -0.18 & \background-color#bad0f8 \color#000000 \text-aligncenter -0.24 & \background-color#ccd9ed \color#000000 \text-aligncenter -0.12 & \background-color#ccd9ed \color#000000 \text-aligncenter -0.12 & \background-color#ccd9ed \color#000000 \text-aligncenter -0.12 & \background-color#d1dae9 \color#000000 \text-aligncenter -0.09 & \background-color#b6cefa \color#000000 \text-aligncenter -0.26 \\
n_pointers & \background-color#cad8ef \color#000000 \text-aligncenter -0.14 & \background-color#c5d6f2 \color#000000 \text-aligncenter -0.17 & \background-color#c3d5f4 \color#000000 \text-aligncenter -0.18 & \background-color#e1dad6 \color#000000 \text-aligncenter 0.04 & \background-color#c3d5f4 \color#000000 \text-aligncenter -0.18 & \background-color#cbd8ee \color#000000 \text-aligncenter -0.13 & \background-color#bad0f8 \color#000000 \text-aligncenter -0.24 & \background-color#cdd9ec \color#000000 \text-aligncenter -0.11 & \background-color#ccd9ed \color#000000 \text-aligncenter -0.12 & \background-color#cad8ef \color#000000 \text-aligncenter -0.14 & \background-color#d4dbe6 \color#000000 \text-aligncenter -0.07 & \background-color#bed2f6 \color#000000 \text-aligncenter -0.22 \\
\end{tabular}
\end{table}


==> implementation.tex <==
%\section{Training a model}






\begin{comment}
    

\subsection{Multi-modal encoding}
As an auxiliary task to improve generalization, we propose the new task of \textbf{generalized multimodal denoising} (as opposed to vanilla multilingual translation), which simplifies concatenation of modalities and allows for modality modifiers (e.g., \texttt{<opt>} for optimized), while not considering all possible concatenations and modifications as different languages. Specifically, we define a canonical sequence encoding that goes as follows:

\texttt{[<c> C </c>] [<s> S </s>] }

where:
\begin{itemize}
    \item C is a function definition in user-level code, in our case, always in C.
    \item S is an assembly function in a given platform, S' is an assembly function definition in another platform, etc. 
    %\item attr is a modifier attribute of the assembly code. In this case, we use \texttt{<opt>} for optimized assembly.
    %\item I is an input example.
    %\item O is an output example
\end{itemize}
All elements between [] brackets are optional. We use special tokens to mark the beginning and end of each modality. In a dataset of C, and assembly, all instances of tuples (C, assembly) are encoded in the same sequence. All elements are optional (e.g., having just C, just C-assembly, etc is fine). Note the ease of adding additional modalities. %Crucially, modifier attributes (opt) are different special tokens, meaning they can be applied to other assembly targets.
\end{comment}

\begin{comment}
\subsection{Multi-modal denoising}
Our goal is to translate. So far, we have just defined how we encode sequences. To translate, generalized multimodal denoising allows masking arbitrary token spans in the input sequence. As other work, but no other work has used that for multi-source/multi-target translation. The first span is replaced by \texttt{<mask:0>}, the second one is replaced by \texttt{<mask:1>}, etc, and the model is trained to predict those spans. For instance:

\begin{figure}
Original:
\begin{lstlisting}[breaklines]

<c> int f(x) {return x+1;} </c> <intel> f: mov... ></intel> </out>
\end{lstlisting}

Sequence input to the model:
\begin{lstlisting}[breaklines]

<c> int f(x) {return <mask:0>} </c> <intel> f: mov...  </intel> 
\end{lstlisting}

Expected out:
\begin{lstlisting}[breaklines]
<mask:0> x+1; <end_of_sequence>
\end{lstlisting}
\caption{Example translation}
\end{figure}
\end{comment}


%\subsubsection{Neural architecture}


.

\begin{comment}
Each input token $a$ is encoded in parallel into
an embedding space and then decoded sequentially. After positional encoding to preserve token order 
the embedding of each token into a combined tensor X depends on its surrounding token embeddings or context.
What context to use is referred to as attention. Each token is mapped to a query vector Q  while its context is mapped to a key Q and value  vector V . The ouptut  vector reprents the new embedding of the token and its context. With single attention the output is the softmax of  a scaled  dotproduct.

$${softmax} (\frac{QK^T}{\sqrt{d}})V$$

With multiple attention we use mulitple attention heads H and later combine them  to give  a new output
Each head $H_i$ is calculated  as


$$h_i= softmax (\frac{Q.W(K.W)^T}{\sqrt{d}})V.W$$

with the new output 

$$ (H_1:H_2:..:H_h) W$$

The output is fed through a dully connected feed forward network that normalises. This is repeated
N times  at which the tokens are now encoded



Decoding applies a similar process except the output tokens, as they are produiceds, are fed into an additional 
multi-headed attention layer. The output of the decoding is a  vector representation of token and context.
This has to be converted into a  distribution over the vocabulary
elements which are then selected based on beam search.
\end{comment}


%\begin{itemize}
    %\item Data (basically, exebench paper)
    %\begin{itemize}
    %    \item function-based. we model entire functions.
    %    \item no duplicates as in anghabench/aiplans
    %    \item consider even the longest instances 
    %    \item larger scale
    %\end{itemize}
    %\item Model itself: a small Transformer trained in the 2 directions. as an auxiliary loss, it also uses partially masked translations. see PLDI overleaf, because it's the same thing
    %\item evaluation:
    %\begin{itemize}
    %    \item datasets: exebench test set, which consists of... and the benchmark used in aiplans, which is a subset of bruce's (64 functions). we use that one to be able to compare with aiplans and because those functions are more "mathematical/compute", but exebench is bigger and more representative
    %    \item baselines: explain baselines. for compilation we use that. for decompilation...
    %    \item metrics and methodology: edit distance, normalized by length and by spaces. io accuracy. we were not able to run some models; for them, we use their reported edit distance, and assume 0 IO accuracy because it's ibvous they can't model functions
    %\end{itemize}
%\end{itemize}


\begin{comment}
\subsection{Dynamic dependency retrieval}


\begin{figure*}
\includegraphics[width=\textwidth]{diagrams/retrieval.pdf}
\caption{
Retrieval
}
\label{fig:retrieval}
\end{figure*}


Our model is trained on code using programmer-defined types,
but to keep training time and cost down, 
we do not ask it to generate definitions for these types.
As a result, our model can hallucinate dependencies that
are defined in other projects, but are not available at
evaluation time for the function in question.
These hallucinations are not necessarily
wrong: most of the time dependencies predicted make sense.
For instance, our model can predict the use of \texttt{my\_int},
a type observed during training that makes sense in the context
it is used in, even if the code really used \texttt{int}.

Hallucinating plausible types without definitions causes evaluation
issues: the code won't compile without the appropriate definition.
Asking the model to generate dependencies makes sequences long and
more difficult to model.  Instead, we \textit{dynamically}
retrieve the dependencies by building an SQL database from the types
in the training.

To differentiate between possible types, we infer type information
over the undefined types used in the implementation.
By recording how a variable is used, we can determine whether it
is an Enum, Struct or primitive, and filter our searches on our
database appropriately.  Using this heuristic drastically reduces
the number of name collisions we have between types and enables
a higher degree of accuracy.


JCW:  Righto --- what are we hoping to convey with the very detailed definition of the way of storing the types lookup database?  Is there an insight we can focus on in writing?
%\begin{comment}
TODO: review writing

A natural shortcoming of function-based code modeling is that the model will learn to use dependencies that are external to the function definition itself, such as user-defined types or auxiliary functions. This is fine if the model predicts the use of dependencies that were actually used in the original C function and are available in evaluation time (e.g., in our train set), but not in the general case, because the model can hallucinate dependencies, as we empirically observed by manually inspecting the model predictions. However, these hallucinations don't have to be necessarily wrong: a key insight is that most of the time the predicted dependencies actually make sense, even if they were not used in the original C function that we are trying to restore by decompiling. For instance, the model can predict the use of "my\_int", a type that it saw during training and that indeed would make perfect sense in the new context, but the original C function actually used "int". 

One solution would be to discard the function-based approach and include all the required dependencies, effectively missing some of the advantages of function-based approaches and making the sequence extremely long and more difficult to model. Instead, we suggest \textit{dynamically retrieving the dependencies}. We build a SQL database from the types used in the train set with the following specifications:

TODO: Explain in words/latex structures instead of code

A dependency (for the queries seen in training):

\begin{verbatim}
@dataclass
class Dep:
    name: str  # symbol name
    kind: str  # func, type or global variable
    actual_type: Optional[str]  # type
    context: str  # pcontents of the file in which was found
    definition: str  # definition of the thing itself
    type_kind: Optional[str] = None  # struct, typedef, enum, or func, only if kind = tpye

    def __post_init__(self):
        assert self.kind in ['func', 'type', 'global_var']

\end{verbatim}

\begin{verbatim}
        sql_create_table = f""" CREATE TABLE IF NOT EXISTS {TABLE} (
                                                       name_plus_type_plus_kind text PRIMARY KEY,
                                                       name text NOT NULL,
                                                       kind text NOT NULL,
                                                       type text,
                                                       context text NOT NULL,
                                                       definition text NOT NULL,
                                                       type_kind text
                                                   ); """
\end{verbatim}


\textbf{}



We iterate over all functions in the train set, and every time there is an external dependency to the function, we insert it in the database, recursively (e.g, if a function calls another function, that's also inserted).

The resulting SQL database, implemented with SQLite, has a size of a few GBs. Then, we build SQL indexes for symbol names, kinds, and types, to be able to query fast in inference.  

In inference, if the model predicts a dependency that wasn't expected, we create a dependency requirement and inject the retrieved dependency, if found. 
\end{comment}

==> new_plots_camready/correlations_ExeBench.tex <==
\begin{table}
\caption{ExeBench feature correlations}
\thnormal
\begin{tabular}{lrrrrrrrrrrrr}
 & \multicolumn{3}{r}{x86_O3} & \multicolumn{3}{r}{x86_O0} & \multicolumn{3}{r}{ARM_O0} & \multicolumn{3}{r}{ARM_O3} \\
 & ChatGPT  & Ghidra  & SLaDe  & ChatGPT  & Ghidra  & SLaDe  & ChatGPT  & Ghidra  & SLaDe  & ChatGPT  & Ghidra  & SLaDe​ \\
compiles & \background-color#f29072 \color#f1f1f1 \text-aligncenter 0.54 & \background-color#d44e41 \color#f1f1f1 \text-aligncenter 0.81 & \background-color#d65244 \color#f1f1f1 \text-aligncenter 0.80 & \background-color#f29274 \color#f1f1f1 \text-aligncenter 0.53 & \background-color#d55042 \color#f1f1f1 \text-aligncenter 0.81 & \background-color#c0282f \color#f1f1f1 \text-aligncenter 0.94 & \background-color#f49a7b \color#000000 \text-aligncenter 0.49 & \background-color#ba162b \color#f1f1f1 \text-aligncenter 0.96 & \background-color#bd1f2d \color#f1f1f1 \text-aligncenter 0.95 & \background-color#ee8669 \color#f1f1f1 \text-aligncenter 0.59 & \background-color#b70d28 \color#f1f1f1 \text-aligncenter 0.98 & \background-color#d85646 \color#f1f1f1 \text-aligncenter 0.78 \\
edit_sim & \background-color#f7ba9f \color#000000 \text-aligncenter 0.32 & \background-color#efcfbf \color#000000 \text-aligncenter 0.16 & \background-color#ee8669 \color#f1f1f1 \text-aligncenter 0.59 & \background-color#f4c6af \color#000000 \text-aligncenter 0.24 & \background-color#dddcdc \color#000000 \text-aligncenter 0.01 & \background-color#f39475 \color#000000 \text-aligncenter 0.53 & \background-color#f1ccb8 \color#000000 \text-aligncenter 0.19 & \background-color#e6d7cf \color#000000 \text-aligncenter 0.07 & \background-color#ef886b \color#f1f1f1 \text-aligncenter 0.58 & \background-color#f4c5ad \color#000000 \text-aligncenter 0.25 & \background-color#ecd3c5 \color#000000 \text-aligncenter 0.13 & \background-color#ee8468 \color#f1f1f1 \text-aligncenter 0.60 \\
asm_length & \background-color#cfdaea \color#000000 \text-aligncenter -0.10 & \background-color#e0dbd8 \color#000000 \text-aligncenter 0.03 & \background-color#cbd8ee \color#000000 \text-aligncenter -0.13 & \background-color#c4d5f3 \color#000000 \text-aligncenter -0.18 & \background-color#d5dbe5 \color#000000 \text-aligncenter -0.06 & \background-color#afcafc \color#000000 \text-aligncenter -0.30 & \background-color#c0d4f5 \color#000000 \text-aligncenter -0.20 & \background-color#cad8ef \color#000000 \text-aligncenter -0.14 & \background-color#a6c4fe \color#000000 \text-aligncenter -0.36 & \background-color#cbd8ee \color#000000 \text-aligncenter -0.13 & \background-color#d8dce2 \color#000000 \text-aligncenter -0.04 & \background-color#c6d6f1 \color#000000 \text-aligncenter -0.16 \\
c_length & \background-color#d3dbe7 \color#000000 \text-aligncenter -0.07 & \background-color#dcdddd \color#000000 \text-aligncenter -0.01 & \background-color#cad8ef \color#000000 \text-aligncenter -0.14 & \background-color#cdd9ec \color#000000 \text-aligncenter -0.11 & \background-color#d8dce2 \color#000000 \text-aligncenter -0.04 & \background-color#bfd3f6 \color#000000 \text-aligncenter -0.21 & \background-color#cedaeb \color#000000 \text-aligncenter -0.11 & \background-color#d6dce4 \color#000000 \text-aligncenter -0.05 & \background-color#bfd3f6 \color#000000 \text-aligncenter -0.21 & \background-color#d1dae9 \color#000000 \text-aligncenter -0.09 & \background-color#dadce0 \color#000000 \text-aligncenter -0.02 & \background-color#c9d7f0 \color#000000 \text-aligncenter -0.15 \\
n_fun_args & \background-color#d2dbe8 \color#000000 \text-aligncenter -0.08 & \background-color#dcdddd \color#000000 \text-aligncenter -0.01 & \background-color#ccd9ed \color#000000 \text-aligncenter -0.12 & \background-color#d3dbe7 \color#000000 \text-aligncenter -0.07 & \background-color#e6d7cf \color#000000 \text-aligncenter 0.07 & \background-color#cbd8ee \color#000000 \text-aligncenter -0.13 & \background-color#d3dbe7 \color#000000 \text-aligncenter -0.07 & \background-color#f2cbb7 \color#000000 \text-aligncenter 0.20 & \background-color#d1dae9 \color#000000 \text-aligncenter -0.09 & \background-color#d2dbe8 \color#000000 \text-aligncenter -0.08 & \background-color#e1dad6 \color#000000 \text-aligncenter 0.04 & \background-color#cfdaea \color#000000 \text-aligncenter -0.10 \\
n_pointers & \background-color#d8dce2 \color#000000 \text-aligncenter -0.04 & \background-color#e0dbd8 \color#000000 \text-aligncenter 0.03 & \background-color#c6d6f1 \color#000000 \text-aligncenter -0.16 & \background-color#d8dce2 \color#000000 \text-aligncenter -0.03 & \background-color#edd1c2 \color#000000 \text-aligncenter 0.14 & \background-color#c5d6f2 \color#000000 \text-aligncenter -0.17 & \background-color#d8dce2 \color#000000 \text-aligncenter -0.04 & \background-color#f2cbb7 \color#000000 \text-aligncenter 0.20 & \background-color#ccd9ed \color#000000 \text-aligncenter -0.12 & \background-color#d5dbe5 \color#000000 \text-aligncenter -0.06 & \background-color#e7d7ce \color#000000 \text-aligncenter 0.08 & \background-color#cad8ef \color#000000 \text-aligncenter -0.14 \\
\end{tabular}
\end{table}


==> new_plots_camready/correlations_Synth.tex <==
\begin{table}
\caption{Synth feature correlations}
\thnormal
\begin{tabular}{lrrrrrrrrrrrr}
 & \multicolumn{3}{r}{ARM_O0} & \multicolumn{3}{r}{ARM_O3} & \multicolumn{3}{r}{x86_O0} & \multicolumn{3}{r}{x86_O3} \\
 & ChatGPT  & Ghidra  & SLaDe  & ChatGPT  & Ghidra  & SLaDe  & ChatGPT  & Ghidra  & SLaDe  & ChatGPT  & Ghidra  & SLaDe​ \\
compiles & \background-color#f59f80 \color#000000 \text-aligncenter 0.48 & \background-color#d65244 \color#f1f1f1 \text-aligncenter 0.80 & \background-color#d0473d \color#f1f1f1 \text-aligncenter 0.84 & \background-color#f7af91 \color#000000 \text-aligncenter 0.39 & \background-color#c12b30 \color#f1f1f1 \text-aligncenter 0.93 & \background-color#e97a5f \color#f1f1f1 \text-aligncenter 0.65 & \background-color#f7aa8c \color#000000 \text-aligncenter 0.41 & \background-color#d44e41 \color#f1f1f1 \text-aligncenter 0.82 & \background-color#d75445 \color#f1f1f1 \text-aligncenter 0.79 & \background-color#f39475 \color#000000 \text-aligncenter 0.53 & \background-color#c12b30 \color#f1f1f1 \text-aligncenter 0.93 & \background-color#e57058 \color#f1f1f1 \text-aligncenter 0.68 \\
edit_sim & \background-color#edd2c3 \color#000000 \text-aligncenter 0.13 & \background-color#efcfbf \color#000000 \text-aligncenter 0.16 & \background-color#f2cab5 \color#000000 \text-aligncenter 0.21 & \background-color#f1ccb8 \color#000000 \text-aligncenter 0.19 & \background-color#f4987a \color#000000 \text-aligncenter 0.50 & \background-color#eed0c0 \color#000000 \text-aligncenter 0.16 & \background-color#efcfbf \color#000000 \text-aligncenter 0.16 & \background-color#e3d9d3 \color#000000 \text-aligncenter 0.05 & \background-color#f4c6af \color#000000 \text-aligncenter 0.24 & \background-color#f1ccb8 \color#000000 \text-aligncenter 0.19 & \background-color#f5c2aa \color#000000 \text-aligncenter 0.26 & \background-color#f7b396 \color#000000 \text-aligncenter 0.36 \\
asm_length & \background-color#d5dbe5 \color#000000 \text-aligncenter -0.06 & \background-color#cfdaea \color#000000 \text-aligncenter -0.09 & \background-color#b6cefa \color#000000 \text-aligncenter -0.27 & \background-color#cfdaea \color#000000 \text-aligncenter -0.10 & \background-color#abc8fd \color#000000 \text-aligncenter -0.32 & \background-color#cedaeb \color#000000 \text-aligncenter -0.11 & \background-color#bcd2f7 \color#000000 \text-aligncenter -0.23 & \background-color#d9dce1 \color#000000 \text-aligncenter -0.02 & \background-color#c6d6f1 \color#000000 \text-aligncenter -0.16 & \background-color#cedaeb \color#000000 \text-aligncenter -0.10 & \background-color#b7cff9 \color#000000 \text-aligncenter -0.25 & \background-color#b5cdfa \color#000000 \text-aligncenter -0.27 \\
c_length & \background-color#cdd9ec \color#000000 \text-aligncenter -0.11 & \background-color#d4dbe6 \color#000000 \text-aligncenter -0.06 & \background-color#b6cefa \color#000000 \text-aligncenter -0.26 & \background-color#e0dbd8 \color#000000 \text-aligncenter 0.03 & \background-color#cbd8ee \color#000000 \text-aligncenter -0.13 & \background-color#cad8ef \color#000000 \text-aligncenter -0.14 & \background-color#c4d5f3 \color#000000 \text-aligncenter -0.17 & \background-color#dcdddd \color#000000 \text-aligncenter -0.00 & \background-color#c1d4f4 \color#000000 \text-aligncenter -0.19 & \background-color#d4dbe6 \color#000000 \text-aligncenter -0.07 & \background-color#c6d6f1 \color#000000 \text-aligncenter -0.16 & \background-color#b5cdfa \color#000000 \text-aligncenter -0.27 \\
n_fun_args & \background-color#c0d4f5 \color#000000 \text-aligncenter -0.20 & \background-color#c1d4f4 \color#000000 \text-aligncenter -0.19 & \background-color#bed2f6 \color#000000 \text-aligncenter -0.22 & \background-color#dadce0 \color#000000 \text-aligncenter -0.02 & \background-color#b6cefa \color#000000 \text-aligncenter -0.27 & \background-color#c4d5f3 \color#000000 \text-aligncenter -0.18 & \background-color#bad0f8 \color#000000 \text-aligncenter -0.24 & \background-color#ccd9ed \color#000000 \text-aligncenter -0.12 & \background-color#ccd9ed \color#000000 \text-aligncenter -0.12 & \background-color#ccd9ed \color#000000 \text-aligncenter -0.12 & \background-color#d1dae9 \color#000000 \text-aligncenter -0.09 & \background-color#b6cefa \color#000000 \text-aligncenter -0.26 \\
n_pointers & \background-color#cad8ef \color#000000 \text-aligncenter -0.14 & \background-color#c5d6f2 \color#000000 \text-aligncenter -0.17 & \background-color#c3d5f4 \color#000000 \text-aligncenter -0.18 & \background-color#e1dad6 \color#000000 \text-aligncenter 0.04 & \background-color#c3d5f4 \color#000000 \text-aligncenter -0.18 & \background-color#cbd8ee \color#000000 \text-aligncenter -0.13 & \background-color#bad0f8 \color#000000 \text-aligncenter -0.24 & \background-color#cdd9ec \color#000000 \text-aligncenter -0.11 & \background-color#ccd9ed \color#000000 \text-aligncenter -0.12 & \background-color#cad8ef \color#000000 \text-aligncenter -0.14 & \background-color#d4dbe6 \color#000000 \text-aligncenter -0.07 & \background-color#bed2f6 \color#000000 \text-aligncenter -0.22 \\
\end{tabular}
\end{table}

